The GAPS Programme at TNG. LXV. Precise density measurement of TOI-1430 b, a young planet with an evaporating atmosphere

Small-sized exoplanets in tight orbits around young stars (10-1000 Myr) give us the opportunity to investigate the mechanisms that led to their formation, the evolution of their physical and orbital properties and, especially, of their atmospheres. Thanks to the all-sky survey carried out by TESS, many of these exoplanets have been discovered and have subsequently been characterized with dedicated follow-up observations. In the context of a collaboration among the GAPS, TKS and CPS teams, we measured with a high level of precision the mass and the radius of TOI-1430 b, a young (~700 Myr) exoplanet with an escaping He atmosphere orbiting the K-dwarf star HD 235088 (TOI-1430). By adopting appropriate stellar parameters, which were measured in this work, we were able to simultaneously model the signals due to strong stellar activity and the transiting planet TOI-1430 b in both photometric and spectroscopic series. This allowed us to measure the density of the planet with high precision, and reconstruct the evolution of its atmosphere. TOI-1430 is an active K-dwarf star born 700+/-150 Myr ago and rotates in ~12 d. It hosts a mini-Neptune whose orbital period is Pb=7.434133+/-0.000004 d. Thanks to long-term monitoring of this target performed with TESS, HARPS-N, HIRES, and APF, we estimated a radius Rb=1.98+/-0.07 $R_{\oplus}$, a mass Mb=4.2+/-0.8 $M_{\oplus}$, and thus a planetary density $\rho$b=0.5+/-0.1 $\rho_{\oplus}$. TOI-1430 b is hence a low-density mini-Neptune with an extended atmosphere, at the edge of the radius gap. Because this planet is known to have an evaporating atmosphere of He, we reconstructed its atmospheric history. Our analysis supports the scenario in which, shortly after its birth, TOI-1430 b may have been super-puffy, with a radius 5x-13x and a mass 1.5x-2x that of today; in ~200 Myr from now, TOI-1430 b should lose its envelope, showing its Earth-size core.

==> table/table1.tex <==
\begin{tabular}{l c c}
\hline
\hline
Parameter     &  TOI-1430 & Reference \\
\hline
\multicolumn{3}{c}{\textit{Other Target Identifiers}} \\
TIC           &     293954617       & (1)\\
2MASS         &   J20022741+5322365 & (2)\\
Gaia~DR3      & 2089570519439964416 & (3)\\
\hline
\multicolumn{3}{c}{\textit{Astrometric information}} \\
$\alpha$(J2016.0)~[deg.]  & 300.61549185196   &   (3)    \\
$\delta$(J2016.0)~[deg.]  & $+$53.37746192023 &   (3)     \\ 
$\mu_{\alpha^{\star}}$~[mas\,yr$^{-1}$] & $165.050\pm0.015$   &     (3)         \\
$\mu_{\delta}$~[mas\,yr$^{-1}$] &  $145.170 \pm 0.015$     &  (3)    \\
Parallax~[mas]  &  $24.2456 \pm 0.0121$ &    (3) \\
Distance~[pc] &   $41.21\pm 0.02$ & (4) \\
RUWE    &    0.966  &  (3) \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hline
\multicolumn{3}{c}{\textit{Photometric information}} \\
$T$~[mag]    & $8.388  \pm      0.006$  & (1)            \\
$G$~[mag]    & $8.953  \pm      0.003$ & (3)        \\
$G_{\rm BP}$~[mag]    & $9.407  \pm      0.003$ & (3)        \\
$G_{\rm RP}$~[mag]    & $8.335  \pm      0.004$ & (3)        \\
%$B$~[mag]    & $ \pm    $   &    (??)          \\
$V$~[mag]    & $ 9.19\pm0.03 $    &   (7) \\
$J$~[mag]    & $7.646\pm 0.037$     & (2)         \\
$H$~[mag]    & $7.224\pm 0.034$ & (2)           \\
$K$~[mag]    & $7.084 \pm 0.016$             & (2)               \\
$W_1$~[mag]  & $6.995 \pm       0.050$  & (5)    \\
$W_2$~[mag]  & $7.095 \pm       0.020$  & (5)              \\
$W_3$~[mag]  & $7.075 \pm       0.016 $ & (5)      \\
$W_4$~[mag]  & $7.160 \pm       0.070$  & (5)        \\
\hline
\multicolumn{3}{c}{\it Fundamental parameters}   \\
RV [\kms]      & $ -27.33\pm 0.13 $    & (3) \\
RV [\kms]      & $ -27.246\pm 0.001 $ & (6)\\
U\ [\kms]      & $-41.728\pm0.023 $    & (8)\\	 	
V\ [\kms]      & $-21.764\pm0.375 $    & (8) \\
W\ [\kms]      & $-18.950\pm0.057 $    & (8)\\
\teff\ (spec.) [K]     &   $5075 \pm 75  $  & Sect. \ref{sec:stellar_parameters}\\
\teff\ (phot.) [K]       &   $5104 \pm 60 $  & Sect. \ref{sec:stellar_parameters}\\  
\logg\ [cgs]                   &   $ 4.55\pm0.05$ & Sect. \ref{sec:stellar_parameters} \\
\feh\ [dex]                    &  $ -0.02\pm0.03$ & Sect. \ref{sec:stellar_parameters} \\
\tih\ [dex]                    &  $0.05\pm0.06$   & Sect. \ref{sec:stellar_parameters} \\
\lstar\ [\lsun]                &  $0.360\pm$0.026 & Sect. \ref{sec:massradius} \\   
\mstar\ [$\mathrm{M_\odot}$]   &  $0.849\pm0.009$ &  Sect. \ref{sec:massradius} \\ %% 
\rstar\ [$\mathrm{R_\odot}$]   &  $0.772\pm0.029$ & Sect. \ref{sec:massradius} \\ %%   
Age [Myr]                      &  $700\pm150$  & Sect. \ref{sec:age} \\ 
$E(B-V)$ [mag]                 &  $0.0022^{+0.0141}_{-0.0022}$  & (9) \\
\vsini\ [\kms]                 & $ 1.9\pm0.6 $ & Sect. \ref{sec:vsini} \\
\prot\ [d]                     & $ 11.9 \pm 0.3 $ & Sect. \ref{sec:rotation} \\
S-index (MW)                    & $ 0.480 \pm 0.006 $  & Sect. \ref{sec:activity} \\
\logrhk\                       & $-4.480\pm 0.003 $  & Sect. \ref{sec:activity}   \\
$\log L_{X}$ [erg s$^{-1}$]    & $ (1.89\pm0.07)\times 10^{28} $  & (10) \\   
$\log L_{X}/L_{bol}$           & $ -4.86\pm0.03 $   & Sect. \ref{sec:activity} \\
$EW_{\rm Li}$ [m\AA]            & $ 0.6 \pm0.2  $ & Sect. \ref{sec:lithium}  \\
A(Li)$_{\rm NLTE}$             & $<0.1$ & Sect. \ref{sec:lithium}  \\
\hline
\end{tabular}
\tablefoot{$^{(1)}$~\tess Input Catalogue v8.2 (\citealt{2018AJ....156..102S}); $^{(2)}$~Two Micron All Sky Survey (2MASS, \citealt{2006AJ....131.1163S}); $^{(3)}$~Gaia~DR3 (\citealt{2023A&A...674A...1G}); $^{(4)}$~\citet{2021AJ....161..147B}; $^{(5)}$~Wide-field Infrared Survey Explorer (WISE, \citealt{2010AJ....140.1868W}); $^{(6)}$~This work; $^{(7)}$~Hipparcos; $^{(8)}$~\citet{smart2021}; $^{(9)}$~\citet{2021A&A...653A..98M}; $^{(10)}$~\citet{orellmiquel2023}}




==> table/table2.tex <==
% Values updated at 28.06.2024
\begin{tabular}{l l l l}
\hline
\hline
Parameter    &  Unit  &    Prior      &       Value   \\
\hline
\multicolumn{4}{c}{{\it TOI-1430 Stellar activity}} \\
Stellar rotational period ($P_{\rm rot}$) & days & $\mathcal{N}(11.9, 0.3)$  &   $12.058_{-0.082}^{+0.084}$ \\
Decay Timescale of activity ($P_{\rm dec}$) & days & $\mathcal{U}(13, 1000)$  &   $41.4_{-7.8}^{+6.6}$ \\
Coherence scale ($w$)  &  & ... &  $0.842_{-0.070}^{+0.085}$ \\
%
Amplitude of the HARPS-N RV signal & m\,s$^{-1}$ & $\mathcal{U}(0.01, 100)$  &   $8.6_{-1.2}^{+1.5}$  \\
HARPS-N RV offset  & m\,s$^{-1}$ & ... &  $-27244.9_{-2.4}^{+2.4}$ \\
Uncorrelated HARPS-N RV jitter   & m\,s$^{-1}$ & ... & $ 2.86_{-0.24}^{+0.25}$  \\
%
Amplitude of the HIRES RV signal & m\,s$^{-1}$ & $\mathcal{U}(0.01, 100)$  &   $7.8_{-1.2}^{+1.5}$  \\
HIRES RV offset  & m\,s$^{-1}$ & ... & $ -0.7_{-2.2}^{+2.2}$ \\
Uncorrelated HIRES RV jitter   & m\,s$^{-1}$ & ... & $ 2.64_{-0.42}^{+0.47}$  \\
%
Amplitude of the APF RV signal & m\,s$^{-1}$ & $\mathcal{U}(0.01, 100)$  &   $7.8_{-5.7}^{+9.6}$  \\
APF RV offset  & m\,s$^{-1}$ & ... & $ -0.3_{-5.7}^{+4.9}$ \\
Uncorrelated APF RV jitter   & m\,s$^{-1}$ & ... & $ 7.2_{-3.1}^{+2.6}$  \\
%
Amplitude of the HARPS-N \logrhk signal &  & ...  & $  0.0254_{-0.0026}^{+0.0031}$ \\
HARPS-N \logrhk offset  &   & ... & $ -4.4768_{-0.0071}^{+0.0070}$ \\
Uncorrelated HARPS-N \logrhk jitter   &  & ... & $ 0.00776_{-0.00079}^{+0.00077}$ \\
%
Amplitude of the HIRES \logrhk signal &  & ...  & $  0.0242_{-0.0026}^{+0.0031}$ \\
HIRES \logrhk offset  &   & ... & $ -4.44890_{-0.0068}^{+0.0067}$ \\
Uncorrelated HIRES \logrhk jitter   &  & ... & $ 0.00443_{-0.00087}^{+0.00083}$ \\
%
Amplitude of the APF \logrhk signal &  & ...  & $  0.030_{-0.012}^{+0.017}$ \\
APF \logrhk offset  &   & ... & $ -4.427_{-0.020}^{+0.019}$ \\
Uncorrelated APF \logrhk jitter   &  & ... & $ 0.0321_{-0.0058}^{+0.0078}$ \\
%
Amplitude of the HARPS-N H$\alpha$ signal &  & ...  & $  0.00367_{-0.00038}^{+0.00045}$ \\
HARPS-N H$\alpha$ offset  &  & ... & $ 0.2478_{-0.0010}^{+0.0010}$ \\
Uncorrelated HARPS-N H$\alpha$ jitter   &  & ... & $ 0.00143_{-0.00013}^{+0.0012}$ \\
%
Amplitude of the HARPS-N BIS signal & m\,s$^{-1}$ & ...  & $  9.6_{-1.4}^{+1.7}$ \\
HARPS-N BIS offset  & m\,s$^{-1}$ & ... & $ 28.0_{-2.7}^{+2.7}$ \\
Uncorrelated HARPS-N BIS jitter   & m\,s$^{-1}$ & ... & $ 3.13_{-0.21}^{+0.23}$\\
%
%Photometric jitter ($\sigma_{\rm jitter}^{\rm LC}$) &  ppm & ... & $292.5 \pm 1.6$ \\
Stellar density ($\rho_\star$) & $\rho_\odot$ & $\mathcal{N}(1.85
, 0.25)$  &   $1.86_{-0.15}^{+0.16}$  \\
\hline
\multicolumn{4}{c}{{\it TOI-1430~b parameters}} \\
Orbital Period ($P_{\rm b}$)     & days   &  $\mathcal{N}(7.43, 0.05)$  & $  7.4341325_{-0.0000044}^{+0.0000042}$ \\
RV semi-amplitude ($K_{\rm b}$) & m\,s$^{-1}$ & $\mathcal{U}(0.01, 10)$ & $1.63_{-0.31}^{+0.31}$ \\
%Impact factor ($b_{\rm b}$)          &        &  ...                &  $0.435_{-0.060}^{+0.051}$ \\
%Planetary-to-stellar-radius ratio ($(R_{\rm P,b}/R_{\star})$) & \% & ... & $2.360_{-0.028}^{+0.028}$ \\
%Mean longitude of the ascending node ($\Omega_{\rm b}$) & deg & ... & $176.584_{-0.030}^{+0.029} $\\
Orbital eccentricity ($e_{\rm b}$)   & deg & ... & 0 (fixed)  \\
%Limb darkening ($u_1$)         &   & $\mathcal{N}(0.47, 0.01)$ & $0.466_{-0.010}^{+0.010}$ \\
%Limb darkening ($u_2$)         &   & $\mathcal{N}(0.14, 0.01)$ & $0.141_{-0.010}^{+0.010}$ \\
%Central time of the first transit ($T_{\rm 0,b}$)      & BJD    &  $\mathcal{U}(2458705, 2458706)$  & $2458705.64614_{-0.00059}^{+0.00062}$ \\
%Semi-major-axis-to-stellar-radius ratio ($(a_{\rm b}/R_{\star})$) &  & ... & $19.71_{-0.54}^{+0.55}$ \\
Orbital Semi-major axis ($a_{\rm b}$) & au & ... & $ 0.07060_{-0.00055}^{+0.00054}$ \\
%Orbital inclination ($i_{\rm b}$)  & deg & ... & $88.74_{-0.19}^{+0.20}$ \\
%Duration of the transit ($T_{\rm 14,b}$)  & hours & ... & $2.673_{-0.018}^{+0.017}$ \\
%Argument of periastron ($\omega_{\rm b}$)   & deg  & ... & 90 (fixed) \\
%Planetary radius ($R_{\rm P,b}$) & ${\rm R_{\oplus}}$ & ... & $1.982_{-0.069}^{+0.072}$  \\
Planetary mass ($M_{\rm P,b}$) & $M_{\oplus}$ & ... & $4.47_{-0.84}^{+0.84}$  \\
Planetary density ($\rho_{\rm b}$) & $\rho_{\oplus}$ & ... & $0.57_{-0.13}^{+0.13}$\\
\hline
\end{tabular}


==> table/table3.tex <==
% Values updated at 09.07.2024
\begin{tabular}{l l l l}
\hline
\hline
Parameter    &  Unit  &    Prior      &       Value   \\
\hline
\multicolumn{4}{c}{{\it TOI-1430 Stellar activity}} \\
Stellar rotational period ($P_{\rm rot}$) & days & $\mathcal{N}(11.9, 0.3)$  &   $12.17_{-0.12}^{+0.12}$ \\
Decay Timescale of activity ($P_{\rm dec}$) & days & $\mathcal{U}(13, 1000)$  &   $26.8_{-1.6}^{+1.9}$ \\
Coherence scale ($w$)  &  & ... &  $0.65_{-0.17}^{+0.17}$ \\
%
HARPS-N RV offset  & m\,s$^{-1}$ & ... &  $-27244.83_{-0.89}^{+0.87}$ \\
Uncorrelated HARPS-N RV jitter   & m\,s$^{-1}$ & ... & $ 3.22_{-0.23}^{+0.24}$  \\
HARPS-N $V_{\rm c}$ & m\,s$^{-1}$ & ... &  $3.51_{-0.49}^{+0.57}$ \\
HARPS-N $V_{\rm r}$ & m\,s$^{-1}$ & ... &  $31.1_{-4.1}^{+4.9}$ \\
%
HIRES RV offset  & m\,s$^{-1}$ & ... & $ 0.49_{-0.83}^{+0.82}$ \\
Uncorrelated HIRES RV jitter   & m\,s$^{-1}$ & ... & $ 3.21_{-0.29}^{+0.32}$  \\
HIRES $V_{\rm c}$ & m\,s$^{-1}$ & ... &  $3.12_{-0.47}^{+0.56}$ \\
HIRES $V_{\rm r}$ & m\,s$^{-1}$ & ... &  $26.3_{-4.0}^{+4.8}$ \\
%
APF RV offset  & m\,s$^{-1}$ & ... & $ -9.3_{-4.1}^{+3.6}$ \\
Uncorrelated APF RV jitter   & m\,s$^{-1}$ & ... & $ 3.8_{-2.0}^{+2.1}$  \\
APF $V_{\rm c}$ & m\,s$^{-1}$ & ... &  $7.0_{-2.4}^{+2.7}$ \\
APF $V_{\rm r}$ & m\,s$^{-1}$ & ... &  $40_{-14}^{+15}$ \\
%
HARPS-N \logrhk offset  &   & ... & $ -4.4792_{-0.0079}^{+0.0078}$ \\
Uncorrelated HARPS-N \logrhk jitter   &  & ... & $ 0.00866_{-0.00063}^{+0.00067}$ \\
HARPS-N $L1_{\rm c}$ &             & ... &  $0.0331_{-0.0038}^{+0.0046}$ \\
%
HIRES \logrhk offset  &   & ... & $ -4.4879_{-0.0075}^{+0.0075}$ \\
Uncorrelated HIRES \logrhk jitter   &  & ... & $ 0.00693_{-0.00066}^{+0.00071}$ \\
HIRES $L1_{\rm c}$ &             & ... &  $0.0318_{-0.0037}^{+0.0044}$ \\
%
APF \logrhk offset  &   & ... & $ -4.454_{-0.017}^{+0.014}$ \\
Uncorrelated APF \logrhk jitter   &  & ... & $ 0.0301_{-0.0048}^{+0.0064}$ \\
APF $L1_{\rm c}$ &             & ... &  $0.034_{-0.010}^{+0.012}$ \\
%
HARPS-N H$\alpha$ offset  &  & ... & $ 0.2471_{-0.0012}^{+0.0012}$ \\
Uncorrelated HARPS-N H$\alpha$ jitter   &  & ... & $ 0.00192_{-0.00012}^{+0.0013}$ \\
HARPS-N $L2_{\rm c}$ &             & ... & $0.00498_{-0.00058}^{+0.00070}$ \\
%
HARPS-N BIS offset  & m\,s$^{-1}$ & ... & $ 28.27_{-0.53}^{+0.50}$ \\
Uncorrelated HARPS-N BIS jitter   & m\,s$^{-1}$ & ... & $ 3.90_{-0.24}^{+0.26}$\\
HARPS-N $B_{\rm c}$ & m\,s$^{-1}$ & ... &  $1.65_{-0.37}^{+0.42}$ \\
HARPS-N $B_{\rm r}$ & m\,s$^{-1}$ & ... &  $-33.5_{-5.4}^{+4.6}$ \\
%
Photometric jitter ($\sigma_{\rm jitter}^{\rm LC}$) &  ppm & ... & $292.5 \pm 1.6$ \\
Stellar density ($\rho_\star$) & $\rho_\odot$ & $\mathcal{N}(1.85
, 0.25)$  &   $1.86_{-0.15}^{+0.16}$  \\
\hline
\multicolumn{4}{c}{{\it TOI-1430~b parameters}} \\
Orbital Period ($P_{\rm b}$)     & days   &  $\mathcal{N}(7.43, 0.05)$  & $  7.4341325_{-0.0000044}^{+0.0000042}$ \\
RV semi-amplitude ($K_b$) & m\,s$^{-1}$ & $\mathcal{U}(0.01, 10)$ & $1.52_{-0.30}^{+0.30}$ \\
Impact factor ($b_{\rm b}$)          &        &  ...                &  $0.435_{-0.060}^{+0.051}$ \\
Planetary-to-stellar-radius ratio ($(R_{\rm P,b}/R_{\star})$) & \% & ... & $2.360_{-0.028}^{+0.028}$ \\
Mean longitude of the ascending node ($\Omega_{\rm b}$) & deg & ... & $176.584_{-0.030}^{+0.029} $\\
Orbital eccentricity ($e_{\rm b}$)   & deg & ... & 0 (fixed)  \\
Limb darkening ($u_1$)         &   & $\mathcal{N}(0.47, 0.01)$ & $0.466_{-0.010}^{+0.010}$ \\
Limb darkening ($u_2$)         &   & $\mathcal{N}(0.14, 0.01)$ & $0.141_{-0.010}^{+0.010}$ \\
Central time of the first transit ($T_{\rm 0,b}$)      & BJD    &  $\mathcal{U}(2458705, 2458706)$  & $2458705.64614_{-0.00059}^{+0.00062}$ \\
Semi-major-axis-to-stellar-radius ratio ($(a_{\rm b}/R_{\star})$) &  & ... & $19.71_{-0.54}^{+0.55}$ \\
Orbital Semi-major axis ($a_{\rm b}$) & au & ... & $ 0.07060_{-0.00055}^{+0.00054}$ \\
Orbital inclination ($i_{\rm b}$)  & deg & ... & $88.74_{-0.19}^{+0.20}$ \\
Duration of the transit ($T_{\rm 14,b}$)  & hours & ... & $2.673_{-0.018}^{+0.017}$ \\
Planetary radius ($R_{\rm P,b}$) & ${\rm R_{\oplus}}$ & ... & $1.982_{-0.069}^{+0.072}$  \\
Planetary mass ($M_{\rm P,b}$) & $M_{\oplus}$ & ... & $4.15_{-0.83}^{+0.83}$  \\
Planetary density ($\rho_{\rm b}$) & $\rho_{\oplus}$ & ... & $0.53_{-0.12}^{+0.12}$\\
\hline
\end{tabular}




==> table/tableB1.tex <==
\begin{tabular}{l l l l}
\hline
\hline
Parameter    &  Unit  &    Prior      &       Value   \\
\hline
\multicolumn{4}{c}{{\it Candidate TOI-1430~c -- Activity modelled through multidimensional GP (case 1)}} \\
Orbital Period ($P_{\rm c}$)     & days   &  $\mathcal{U}(0.4, 100.0)$  & $  96.4_{-1.1}^{+1.1}$ \\
Semi-major-axis-to-stellar-radius ratio ($(a_{\rm c}/R_{\star})$) &  & ... & $108.5_{-4.1}^{+4.4}$ \\
Orbital Semi-major axis ($a_{\rm c}$) & au & ... & $ 0.3897_{-0.0043}^{+0.0043}$ \\
RV semi-amplitude ($K_{\rm c}$) & m\,s$^{-1}$ & $\mathcal{U}(0.01, 10)$ & $1.27_{-0.33}^{+0.32}$ \\
Orbital eccentricity ($e_{\rm c}$)   & deg & ... & 0 (fixed)  \\
Mean longitude of the ascending node ($\Omega_{\rm c}$) & deg & ... & $289_{-31}^{+30} $\\
Planetary mass ($M_{\rm P,c} \sin{i_{\rm c}}$) & $M_{\oplus}$ & ... & $8.2_{-2.1}^{+2.1}$  \\
\hline
\multicolumn{4}{c}{{\it Candidate TOI-1430~c -- Activity modelled through multidimensional GP (case 2)}} \\
Orbital Period ($P_{\rm c}$)     & days   &  $\mathcal{U}(0.4 ,20.0)$  & $  12.685_{-0.015}^{+0.015}$ \\
Semi-major-axis-to-stellar-radius ratio ($(a_{\rm c}/R_{\star})$) &  & ... & $28.1_{-1.0}^{+1.1}$ \\
Orbital Semi-major axis ($a_{\rm c}$) & au & ... & $ 0.10079_{-0.0081}^{+0.0080}$ \\
RV semi-amplitude ($K_{\rm c}$) & m\,s$^{-1}$ & $\mathcal{U}(0.01, 10)$ & $1.65_{-0.40}^{+0.39}$ \\
Orbital eccentricity ($e_{\rm c}$)   & deg & ... & 0 (fixed)  \\
Mean longitude of the ascending node ($\Omega_{\rm c}$) & deg & ... & $164_{-31}^{+32} $\\
Planetary mass ($M_{\rm P,c} \sin{i_{\rm c}}$) & $M_{\oplus}$ & ... & $5.4_{-1.3}^{+1.3}$  \\
\hline
\multicolumn{4}{c}{{\it Candidate TOI-1430~c -- Activity modelled through quasiperiodic GP}} \\
Orbital Period ($P_{\rm c}$)     & days   &  $\mathcal{U}(0.4, 100.0)$  & $  13.267_{-0.016}^{+0.016}$ \\
Semi-major-axis-to-stellar-radius ratio ($(a_{\rm c}/R_{\star})$) &  & ... & $28.9_{-1.1}^{+1.1}$ \\
Orbital Semi-major axis ($a_{\rm c}$) & au & ... & $ 0.10385_{-0.00083}^{+0.00081}$ \\
RV semi-amplitude ($K_{\rm c}$) & m\,s$^{-1}$ & $\mathcal{U}(0.01, 10)$ & $2.47_{-0.50}^{+0.50}$ \\
Orbital eccentricity ($e_{\rm c}$)   & deg & ... & 0 (fixed)  \\
Mean longitude of the ascending node ($\Omega_{\rm c}$) & deg & ... & $108_{-23}^{+23} $\\
Planetary mass ($M_{\rm P,c} \sin{i_{\rm c}}$) & $M_{\oplus}$ & ... & $8.2_{-1.7}^{+1.7}$  \\
\hline
\end{tabular}

==> table/tableD1.tex <==
\begin{tabular}{l c c l c c l c c}
\hline
\hline
Telescope    &  $T_0$ [BJD$_{\rm TDB}-2457000.0$] &    $R_{\rm P,b}/R_\star$  & Telescope    &  $T_0$ [BJD$_{\rm TDB}-2457000.0$] &    $R_{\rm P,b}/R_\star$ & Telescope    &  $T_0$ [BJD$_{\rm TDB}-2457000.0$] &    $R_{\rm P,b}/R_\star$  \\
\hline 
TESS   &      $1683.3416_{-0.0130}^{+0.0040}$ & $0.0225_{-0.0032}^{+0.0029}$ &  TESS   &      $2441.6286_{-0.0032}^{+0.0024}$ & $0.0245_{-0.0013}^{+0.0012}$ & TESS   &      $2850.5030_{-0.0023}^{+0.0018}$ & $0.0258_{-0.0013}^{+0.0012}$ \\        
TESS   &      $1690.7768_{-0.0025}^{+0.0020}$ & $0.0251_{-0.0023}^{+0.0021}$ &  TESS   &      $2776.1629_{-0.0021}^{+0.0027}$ & $0.0212_{-0.0015}^{+0.0014}$ & TESS   &      $3341.1541_{-0.0019}^{+0.0024}$ & $0.0224_{-0.0015}^{+0.0014}$ \\        
TESS   &      $1698.2116_{-0.0010}^{+0.0012}$ & $0.0263_{-0.0027}^{+0.0028}$ &  TESS   &      $2783.5952_{-0.0040}^{+0.0024}$ & $0.0224_{-0.0013}^{+0.0013}$ & TESS   &      $3348.5882_{-0.0026}^{+0.0040}$ & $0.0221_{-0.0012}^{+0.0012}$ \\        
TESS   &      $1705.6493_{-0.0017}^{+0.0028}$ & $0.0241_{-0.0013}^{+0.0013}$ &  TESS   &      $2791.0289_{-0.0015}^{+0.0014}$ & $0.0268_{-0.0016}^{+0.0015}$ & TESS   &      $3356.0249_{-0.0071}^{+0.0020}$ & $0.0243_{-0.0015}^{+0.0014}$ \\        
TESS   &      $1713.0824_{-0.0032}^{+0.0046}$ & $0.0225_{-0.0012}^{+0.0012}$ &  TESS   &      $2798.4652_{-0.0019}^{+0.0014}$ & $0.0230_{-0.0015}^{+0.0014}$ & TESS   &      $3363.4558_{-0.0030}^{+0.0048}$ & $0.0255_{-0.0015}^{+0.0014}$ \\        
TESS   &      $1720.5170_{-0.0019}^{+0.0025}$ & $0.0210_{-0.0014}^{+0.0013}$ &  TESS   &      $2805.8974_{-0.0015}^{+0.0016}$ & $0.0211_{-0.0012}^{+0.0012}$ & TESS   &      $3370.8904_{-0.0015}^{+0.0014}$ & $0.0272_{-0.0014}^{+0.0013}$ \\        
TESS   &      $1727.9512_{-0.0041}^{+0.0070}$ & $0.0228_{-0.0014}^{+0.0013}$ &  TESS   &      $2813.3340_{-0.0024}^{+0.0020}$ & $0.0241_{-0.0013}^{+0.0013}$ & TESS   &      $3378.3251_{-0.0012}^{+0.0013}$ & $0.0283_{-0.0013}^{+0.0012}$ \\        
TESS   &      $1735.3817_{-0.0012}^{+0.0015}$ & $0.0247_{-0.0016}^{+0.0015}$ &  TESS   &      $2820.7653_{-0.0015}^{+0.0016}$ & $0.0245_{-0.0015}^{+0.0014}$ & TESS   &      $3385.7572_{-0.0014}^{+0.0020}$ & $0.0247_{-0.0013}^{+0.0012}$ \\        
TESS   &      $1742.8169_{-0.0016}^{+0.0026}$ & $0.0232_{-0.0014}^{+0.0013}$ &  TESS   &      $2828.1993_{-0.0020}^{+0.0013}$ & $0.0241_{-0.0013}^{+0.0012}$ & TESS   &      $3393.1947_{-0.0013}^{+0.0013}$ & $0.0243_{-0.0011}^{+0.0011}$ \\        
TESS   &      $1757.6821_{-0.0020}^{+0.0029}$ & $0.0249_{-0.0014}^{+0.0013}$ &  TESS   &      $2835.6361_{-0.0015}^{+0.0036}$ & $0.0249_{-0.0013}^{+0.0013}$ & LCO/1.0m~McDonald   & $2359.8571_{-0.0049}^{+0.0096}$ & $0.0296_{-0.0014}^{+0.0013}$ \\
TESS   &      $2426.7581_{-0.0022}^{+0.0016}$ & $0.0256_{-0.0014}^{+0.0014}$ &  TESS   &      $2843.0699_{-0.0032}^{+0.0025}$ & $0.0210_{-0.0013}^{+0.0012}$ & LCO/1.0m~Teide      & $2798.4662_{-0.0039}^{+0.0048}$ & $0.0233_{-0.0013}^{+0.0013}$ \\
TESS   &      $2434.1877_{-0.0032}^{+0.0038}$ & $0.0222_{-0.0013}^{+0.0013}$ &         &                                                             &        &                 \\
\hline
\end{tabular}

